DeFiGuard: A Price Manipulation Detection Service in DeFi using Graph Neural Networks

The prosperity of Decentralized Finance (DeFi) unveils underlying risks, with reported losses surpassing 3.2 billion USD between 2018 and 2022 due to vulnerabilities in Decentralized Applications (DApps). One significant threat is the Price Manipulation Attack (PMA) that alters asset prices during transaction execution. As a result, PMA accounts for over 50 million USD in losses. To address the urgent need for efficient PMA detection, this paper introduces a novel detection service, DeFiGuard, using Graph Neural Networks (GNNs). In this paper, we propose cash flow graphs with four distinct features, which capture the trading behaviors from transactions. Moreover, DeFiGuard integrates transaction parsing, graph construction, model training, and PMA detection. Evaluations on a dataset of 208 PMA and 2,080 non-PMA transactions show that DeFiGuard with GNN models outperforms the baseline in Accuracy, TPR, FPR, and AUC-ROC. The results of ablation studies suggest that the combination of the four proposed node features enhances DeFiGuard's efficacy. Moreover, DeFiGuard classifies transactions within 0.892 to 5.317 seconds, which provides sufficient time for the victims (DApps and users) to take action to rescue their vulnerable funds. In conclusion, this research offers a significant step towards safeguarding the DeFi landscape from PMAs using GNNs.

==> sections/bios.tex <==
% \vskip 0pt plus -1fil
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pdf/bio_dabao.png}}]{Dabao Wang} received a Bachelor degree in Computer Science (with an Honors degree) from Monash University. 
% He is currently working towards a PhD in the Department of Software Systems and Cybersecurity of the Faculty of Information Technology at Monash University. Dabao is interested in all aspects of security with a focus on the security of smart contracts, and decentralized finance (DeFi) security.
% \end{IEEEbiography}
% \vskip -1\baselineskip plus -1fil

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pdf/bio_bang.jpg}}]{Bang Wu} received a Ph.D. from the Faculty of Information Technology, Monash University, Australia. His research interests include trustworthy graph-based machine learning, trustworthy machine learning on multimodal systems, and various facets of security and privacy in machine learning across different domains. 
% \end{IEEEbiography}
% \vskip -1\baselineskip plus -1fil

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pdf/bio_xyuan.jpg}}]{Xingliang Yuan} is currently a senior lecturer (aka U.S. associate professor) with the Department of Software Systems and Cybersecurity, Faculty of Information Technology, Monash University, Australia. He has authored or coauthored in prestigious venues in cybersecurity, computer networks, and distributed systems, including ACM CCS, NDSS, IEEE INFOCOM, IEEE Transactions on Dependable and Secure Computing, IEEE Transactions on Information Forensics and Security, and IEEE Transactions on Parallel and Distributed Systems. His research interests include data security and privacy, secure networked system, machine learning security and privacy, and confidential computing. His research has been supported by Australian Research Council, CSIRO Data61, and Oceania Cyber Security Centre. He was the recipient of Dean’s Award for Excellence in Research by an Early Career Researcher at Monash Faculty of IT in 2020, the Best Paper Award in European Symposium on Research in Computer Security (ESORICS) 2021, the IEEE Conference on Dependable and Secure Computing (IDSC) 2019, and the IEEE International Conference on Mobility, Sensing and Networking (MSN) 2015.
% \end{IEEEbiography}
% \vskip -1\baselineskip plus -1fil


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pdf/bio_leiwu.pdf}}]{Lei Wu} is an Associate Professor with the School of Cyber Science and Technology, and the College of Computer Science and Technology, Zhejiang University, China. He obtained his Ph.D. degree from North Carolina State University in 2015. His research interest lies mainly in security areas, including system security and blockchain security.
% \end{IEEEbiography}
% \vskip -1\baselineskip plus -1fil

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pdf/bio_yajinzhou.pdf}}]{Yajin Zhou} received the Ph.D. degree in computer science from North Carolina State University, Raleigh, NC, USA. He is currently a ZJU 100 Young Professor with the School of Cyber Science and Technology, and the College of Computer Science and Technology, Zhejiang University, China. His research mainly focuses on smartphone and system security, such as identifying real-world threats and building practical solutions, mainly in the context of embedded systems (or IoT devices).
% \end{IEEEbiography}
% \vskip -1\baselineskip plus -1fil


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pdf/bio_helei.jpeg}}]{Helei Cui} received the B.E. degree in Software Engineering from Northwestern Polytechnical University, in 2010, the M.S. degree in Information Engineering from The Chinese University of Hong Kong, in 2013, and the Ph.D. degree in Computer Science from the City University of Hong Kong, in 2018. He is currently a Professor with the School of Computer Science, Northwestern Polytechnical University, China. His research interests include Industrial Internet of Things, Privacy-Preserving Computing, Secure Deduplication, Decentralized Cloud Storage, etc.
% \end{IEEEbiography}


==> sections/cfg.tex <==
\section{Cash Flow Graph}
\label{sec:cfg}
\fixme{Could be updated once more explanation about why using graph to and GNNs for analysis. (Recall that graph representing the cash flow can include sufficient information for malicious actions? And then introduce what is our graph and what information is included in this graph (to satisfy requirements)).} 
Through exploring both malicious and benign EVM-based transactions, we have determined that EVM-based transactions can be represented as cash flow graphs. 
In this section, we start by introducing some terminologies to favor readability.
Then, we reveal more details regarding the edge and node utilized to construct the cash flow graph.
Finally, we elaborate on an illustrative example for ease of understanding the cash flow graph.

\subsection{Notations}
To favor the readability, we summarize a list of notations.
\begin{description}[leftmargin=10pt]
    \item[Node \term{V}:] 
    The node in the graph represents an account sending or receiving assets.
    Specifically, \term{V} is a set of nodes identified in a transaction (see more details in Section~\ref{subsec:node}).
    In this study, we further differentiate nodes based on their type (i.e., EOA or CA) and transparency.
    \item[Edges \term{E}:]
    The edge in the graph represents the asset transfer in terms of the native token and the ERC20 token.
    Specifically, \(\mathcal{E} \subseteq  (\mathcal{V}\) X \(\mathcal{V})\) is a set of directed edges extracted from a transaction (see more details in Section~\ref{subsec:edge}).
    \item[Node Feature \term{X}:]
    Node feature \term{X} denotes a set of features extracted from the graph metadata \(\mathcal{K}\) consisting of \(\mathcal{K}^{V} \) and \(\mathcal{K}^{E}\), where \(\mathcal{K}^{V}\) denotes nodes' metadata and \(\mathcal{K}^{E}\) denotes edges' metadata, by the feature function \(\lambda\).
    The feature function \(\lambda\) is a function aiming to extract and normalize the feature \(x\ \epsilon \ \mathcal{X}\) for a node \(v\ \epsilon\ \mathcal{V}\) based on the graph metadata \(\mathcal{K}\).
    Specifically, \(\lambda : (\mathcal{K}^{V}, \mathcal{K}^{E}) \rightarrow \mathcal{X}\) takes \(\mathcal{K}^{V}\) and \(\mathcal{K}^{E}\) as inputs and outputs a feature set \(\mathcal{X}\).
    \item[Cash Flow Graph \term{G}:]
    The cash flow graph \(\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{X})\) is a graph that represents the asset transfer information within a transaction (see more details in Section~\ref{subsec:example}).
\end{description}




\subsection{Node}
\label{subsec:node}
\new{
    Each node in the cash flow graph represents an address sending and receiving assets.
    In particular, there are two categories of addresses used in EVM-based blockchain systems: {\it External Owned Addresses} and {\it Contract Addresses}.
    Within a transaction, the CA is passively triggered to transfer assets based on the transaction's input data. 
    Distinguishing the type of each node can help the classifier learn the behavior pattern in terms of different nodes.
    % 
    As for the node's metadata, the type of the node will be distinguished and attached as metadata for each extracted node.
}

% An External Owned Address (aka. EOA) is controlled by the private key owned by one or a group of users. 
% To interact with other addresses (e.g., to transfer assets), an EOA needs to send a transaction to the blockchain network with specified input data (e.g., the value of ether to send).
% In contrast, a Contract Address (aka. CA) is controlled by the smart contract (known as snippets of JavaScript-like code) and can be created by an EOA or another CA.
% Creating a CA requires the creator to send a transaction to deploy the smart contract, which will be attached to the CA.
% Based on the business logic assigned in the smart contract, CAs can serve different purposes and be further categorized into different classes such as token contracts, proxy contracts, and storage contracts (more details in Section~\ref{subsec:graph_builder}).

\subsection{Edge}
\label{subsec:edge}
\new{
    The edges \term{E} in the cash flow graph \term{G} indicate the directive asset transfer from the sending account to the receiving account.
    % 
    Given the fact that the native token and ERC20 token transfers are dominating the token trading ecosystem in EVM-based blockchain, 
    in this paper, we consider these two types of token transfers in our graph construction process.
    Based on the data presented by the CoinMarketCap~\footnote{CoinMarketCap is one of the most famous statistical websites for cryptocurrencies}~\cite{coinmarketcap}, the majority (over 80\%) of market capability is covered by 100 different tokens.
    % 
    As for the edge's metadata, each extracted edge will contain the information including the sender node, receiver node, transferred asset, and transferred amount.
}

% Specifically, the native token (such as Ether or ETH in the Ethereum network) is a crucial component of the EVM-based blockchain network and plays a vital role as the transaction fee and the incentive for minders.
% % 
% As for the ERC20 token, it is a templated and customizable token, which not only provides basic functionality (e.g., transfer between accounts) but also allows the developer to add their customized logic.
% For example, many {\dapp}s (e.g., Uniswap~\cite{UniswapV2} and Compound~\cite{compound}) utilize the ERC20 standard token as the main component to embed their business logic.
% As the ERC20 token allows users to use their tokens in other \dapp (such as decentralized exchange, lending, etc.), it rapidly becomes one of the most popular crypto assets that boost the prosperity of the DeFi ecosystem.



\subsection{Illustrative Example}
\label{subsec:example}
\input{tex_figures/3_cash_flow_graph.tex}
For ease of understanding the cash flow graph, we provide an example in Figure~\ref{fig:cash_flow_graph} presenting a cash flow graph converted from a transaction based on asset transfers. There are 5 distinct nodes (including 2 EOAs and 3 CAs) and 7 edges (including native token and ERC20-standard token transfers). 
Specifically, in this cash flow graph, \textit{EOA}-1 starts transferring {\bf 0.1 ETH} to the Contract Address \textit{CA}-1. Then, the \textit{CA}-1 performs a swap-like transfer for the received {\bf 0.1 ETH} with \textit{CA}-2 and transfers {\bf 120 USDT} to \textit{EOA}-2. With the received {\bf 120 USDT}, \textit{EOA}-2 also performs a swap-like transfer with \textit{CA}-3 and received {\bf 0.11 ETH}. Finally, \textit{EOA}-2 transfers 0.11 ETH to \textit{EOA}-1.
%
By converting the transaction into the cash flow graph, the semantic information can be refined from raw transaction data and clearly represented as a graph. 
In this case, with the help of asset type and amounts recorded in the edges, we can predict that the transaction is performing an arbitrage-like action by comparing transfer pairs (\encircled{2}, \encircled{3}) and (\encircled{5}, \encircled{6}). Moreover, the profit of each node can be calculated to provide more comprehensive information to identify malicious transactions.




==> tex_algorithm/5_feature_extractor.tex <==
\begin{algorithm}
\caption{Feature Extractor \(\lambda\)}
\begin{algorithmic} 
\REQUIRE $Information\ \mathcal{I}: \mathcal{I}_{v} \cup \mathcal{I}_{e}$
\ENSURE $Feature\ Set\ \mathcal{X}$
\STATE $y \gets 1$
\STATE $y \gets 1$
\IF{$n < 0$}
\STATE $X \gets 1 / x$
\STATE $N \leftarrow -n$
\ELSE
\STATE $X \leftarrow x$
\STATE $N \leftarrow n$
\ENDIF
\WHILE{$N \neq 0$}
\IF{$N$ is even}
\STATE $X \leftarrow X \times X$
\STATE $N \leftarrow N / 2$
\ELSE[$N$ is odd]
\STATE $y \leftarrow y \times X$
\STATE $N \leftarrow N - 1$
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> tex_equations/4_gc_inference.tex <==
\begin{equation}
\label{eq:gc_inference}
\begin{aligned}
    f_{gc\_inference}(\mathcal{G}_{u}s, \mathcal{F}) = \mathcal{P},\ where\ \mathcal{P} \rightarrow 0\ or\ 1 
\end{aligned}
\end{equation} 

==> tex_equations/4_profit.tex <==
\begin{equation}
\label{eq:profit}
\begin{aligned}
    p = \mathcal{F}
\end{aligned}
\end{equation} 

==> tex_equations/5_fpr.tex <==
\begin{equation}
\label{eq:fpr}
\begin{aligned}
FPR = \frac{FP}{FP + TN}
\end{aligned}
\end{equation} 

==> tex_equations/5_gmean.tex <==
\begin{equation}
\label{eq:gmean}
\begin{aligned}
% \mathbf{m}_{v}^{(t)}&=\sum_{u\in\mathcal{N}(v)}M_{t}(\mathbf{h}_u^{(t-1)},\mathbf{h}_v^{(t-1)}, \mathbf{e}_{uv}), \\
% \mathbf{h}_v^{(t)} &= U_t(\mathbf{h}_v^{(t-1)}, \mathbf{m}_v^{(t)}),
\end{aligned}
\end{equation} 

==> tex_equations/5_tpr.tex <==
\begin{equation}
\label{eq:tpr}
\begin{aligned}
TPR = \frac{TP}{TP + FN}
\end{aligned}
\end{equation} 

==> tex_figures/4_call_trace.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1\linewidth]{pdf/4_call_trace.pdf}
    \caption{\bf The call trace of a transaction.} 
    \label{fig:call_trace}
\end{figure}

==> tex_tables/experiments.tex <==
\begin{table*}[h!]
    % \caption{The Distribution of Users in Different Risk Levels.}
    \caption{\bf Performance comparison.}
 	\label{tbl:datacollection}
	\centering
% 	\resizebox{1\textwidth}{!}{
    \begin{tabular}{ccccccc}
		\toprule
		\multirow{2}{*}{Time Range} & \multicolumn{3}{c}{Malicious Transactions} & \multicolumn{3}{c}{Honest Transactions} \\
% 		\midrule
		& Internal Transaction & Transfer Count & Token Count & Internal Transaction & Transfer Count & Token Count\\
		\midrule
		2020-01-01 & 25(Avg) & 40(Avg) & 3(Avg)&25(Avg) & 40(Avg) & 3(Avg)\\
		to & 25(Max) & 40(Avg) & 3(Max)&25(Max) & 40(Max) & 3(Max)\\
		2022-01-01 & 25(Min) & 40(Min) & 3(Min) &25(Min) & 40(Min) & 3(Min)\\
		\midrule
		Total & \multicolumn{3}{c}{30} & \multicolumn{3}{c}{100} \\
		\bottomrule
 	\end{tabular}
%  	}
\end{table*}

==> tex_tables/real_time_performance.tex <==
\begin{table}[h!]
    \caption{\bf The real-time performance of {\tool}.}
 	\label{tbl:performance}
	\centering
% 	\resizebox{1\textwidth}{!}{
    \begin{tabular}{ccccc}
		\toprule
		Model & Acc(\%) & Prec(\%) & Recall(\%) & F1(\%) \\
		\midrule
	      % GCN (Node) & 87.8 & 52.0 & 34.7 & 38.5\\
            MLP & N/A & N/A & N/A & N/A\\
		GCN & 98.4 & 94.1 & 99.5 & 96.5\\
            GraphSAGE & N/A & N/A & N/A & N/A\\
  
	    % \midrule
	    % \multirow{2}{*}{Invocation} & GCN-Node & - & - & - & - \\
	    % & GCN-Graph & - & - & - & - \\
        \bottomrule
 	\end{tabular}
%  	}
\end{table}
